On-Device Training of Fully Quantized Deep Neural Networks on Cortex-M Microcontrollers

On-device training of DNNs allows models to adapt and fine-tune to newly collected data or changing domains while deployed on microcontroller units (MCUs). However, DNN training is a resource-intensive task, making the implementation and execution of DNN training algorithms on MCUs challenging due to low processor speeds, constrained throughput, limited floating-point support, and memory constraints. In this work, we explore on-device training of DNNs for Cortex-M MCUs. We present a method that enables efficient training of DNNs completely in place on the MCU using fully quantized training (FQT) and dynamic partial gradient updates. We demonstrate the feasibility of our approach on multiple vision and time-series datasets and provide insights into the tradeoff between training accuracy, memory overhead, energy, and latency on real hardware.

==> sections/rebuttal.tex <==
\newpage
\section{Responses to Reviewer Comments}

\subsection{General Response}

\noindent\blue{Dear Reviewers,}

\blue{Thank you very much for your careful review of our manuscript and for the constructive feedback. We revised the manuscript according to your questions and suggestions as follows.}   

\blue{A common request raised is to provide a qualitative comparison with the state of the art and in particular~\cite{lin2022device}. To address this concern, we have replicated the experiments performed by Lin et al.~\cite{lin2022device} for their optimizer SGD+M+QAS and their DNN architecture MCUNet-5FPS~\cite{lin2020mcunet} using our framework and methods presented in this paper. In the new added Sec.~\ref{sec:evaluation:mcunet}, we provide a comparison of our optimizer with the results of SGD+M+QAS, which Lin. et al~\cite{lin2022device} show in Table 1, and a discussion of result. There it is also shown that our method is able to match closely, and in many cases even exceed, the retraining performance of SGD+M+QAS. The results further show that, unlike~\cite{lin2022device}, our method is not limited to a single CNN architecture, i.e., MBedNet, but can be applied to many common CNN architectures, like MCUNet-5FPS, without any code changes. Moreover, Lin et al.~\cite{lin2022device} do not provide any detailed memory and latency results for their experiments in Table 1. Therefore, in Sec.~\ref{sec:evaluation:mcunet} we additionally discuss memory utilization and latency of MCUNet-5FPS compared to MBedNet, the DNN we used in our experiments, in the context of our framework. The additional experiments show that MBedNet is a DNN architecture more suitable for on-device training compared to MCUNet, as it has similar retraining capabilities while requiring significantly less memory and computational time to run. Specifically, Lin et al.~\cite{lin2022device} state that inference, not including training, of their DNN can be performed at about 5FPS (200 ms per sample) on most Cortex-M7 MCUs, see the left light blue bar in Fig.~\ref{fig:mcunet_vs_mbednet}. However, our results in Sec.~\ref{sec:evaluation:mcunet} show that with MBedNet and for the same data set, not only inference but also training, i.e. backpropagation, can be performed below 200 ms, see the right bar in Fig.~\ref{fig:mcunet_vs_mbednet}. In summary, we believe that the additional experiments and comparisons provided allow for a better assessment of the effectiveness of our method in the context of the current state-of-the-art.}

\blue{Below, we provide more specific answers to all questions. We have marked all new or revised parts in blue throughout the manuscript.}

\noindent\blue{\\Best regards,\\The Authors}

\subsection{Review \#51A}

\textit{"Fully quantized on-device training (FQT) is not new, it has been used in many other works."}

\blue{Indeed, FQT has been discussed in the literature before. However, except for~\cite{lin2022device}, we are not aware of any large-scale quantitative results for on-device FQT on MCUs. To our knowledge, FQT is usually discussed either from a theoretical perspective, focusing only on limited learning and weight updating strategies, or for larger embedded platforms such as mobile. In contrast, considering full training of arbitrary CNN architectures, as presented in this work, both the resource constraints and the strict computational budget present on Cortex-M MCUs require a careful and deliberate selection of memory and latency-preserving techniques to meet system constraints and make on-device training feasible. As a result, this work investigates techniques, one of which is FQT, used during the presented exploration of the multi-objective tradeoff that arises in the application of DNN training on Cortex-M MCUs, and which, to the best of our knowledge, has not been widely discussed or evaluated in the literature.}
    
\textit{"No comparaison is done with SOTA. The authors mentionned for instance that [10] is one of the closest work, but the don't compare the performances of the two methods."}

\blue{We agree with the reviewer and are thankful for pointing this out. Therefore, we made the effort to provide additional comparative experiments of our approach with SGD+M+QAS~\cite{lin2022device} for MCUNet-5FPS and present these new results in Sec.~\ref{sec:evaluation:mcunet}. The additional experiments show that our optimizer slightly surpasses the performance of SGD+M+QAS for retraining MCUNet, and that our DNN architecture MBedNet is more suitable for on-device training compared to MCUNet, as it has similar retraining capabilities while requiring significantly less memory and computational time to run.}
    
\textit{"the authors claim that "our method focuses on general CNN support for different domains and applications" but they tested the method only on 1 DNN architecture (MbedNet)."}

\blue{Our method infers the BP graph automatically based on the structure of the DNN's forward pass and emits additional code accordingly during the initial offline mapping/lowering of the DNN to C code. This BP graph inference process is based on the chain-rule and works to the same principles as other "autograd" features of other DNN training frameworks like Pytorch or Tensorflow. As a result, like in Pytorch or Tensorflow, training of any CNN is possible out-of-the-box as long as the partial derivatives are implemented for all layer types the CNN consists of (and memory constraints of the target system the training should be conducted on are met). For example, in the additional experiments presented in Sec.~\ref{sec:evaluation:mcunet}, we could directly retrain MCUNet-5FPS because all of its layer types were already supported by our codebase for training.}
    
\textit{"More discussions ont eh experimental results are needed. For example we don't understand why in fig 4.A and "animals Dataset" "Mixed " gives better results than baseline. Same for figure 5.B for nrf52840 (M4), why mixed consumes less energy than uint8."}

\blue{A general observation that can be made with quantized DNNs is that after quantization, their performance on the test dataset can slightly improve while it can worsen on the training dataset. As you sharply noticed, in our results, this effect can be seen, for example, in Fig.~\ref{fig:retrain_results:accuracy} for the animal dataset and the mixed configuration, but it can also be seen, for example, in the results of~\cite{lin2022device}. A common explanation for the occurrence of this effect is that the error introduced by quantization can sometimes eliminate overfitting effects introduced by the original floating-point training, resulting in a slightly better abstraction of the DNN and thus improved performance on unseen test data.}

\blue{We believe the small differences in energy between the uint8 and mixed configurations in Fig.~\ref{fig:compare:energy} to be a result of the classification head being computed in floating-point instead of a quantized data format. The main advantage of quantizing the layers of a DNN, besides saving memory, is that on Cortex-M MCUs, SIMD instructions from ARM's DSP extension can be used for integer types that are not available for floating-point data types. However, this comes at the cost of introducing additional arithmetic operations, as values must be both quantized and dequantized during the computation of the DNN, see, for example, Eq.~\eqref{eq:backward_pass_err_quant}. As a result, from both a latency and energy point of view, this quantization tradeoff becomes particularly advantageous for layers with many weights and large feature maps, where the benefits of data parallelism can be exploited heavily, but may become unfavorable for small layers, such as the last linear layers of a CNN, where the overhead of computing the additional quantization and dequantization operations may be higher than the energy and latency saved by using the SIMD instructions. Therefore, we argue that computing the last layers in floating-point while keeping all the other more expensive convolutional layers quantized, as we do in the mixed configuration, may in some cases result in a more favorable tradeoff from both an energy and latency perspective, leading to the results that can be seen both in Fig.~\ref{fig:compare:latency} and~\ref{fig:compare:energy}.}

\subsection{Review \#51B}

\textit{"The authors mention that reference [10] is the closest prior work. Among the limitations listed in Sec II are that [10] is only optimized for a specific DNN architecture, and that statically fixing the gradients to be updated at compile time is suboptimal. While both are valid points, they are not supported by comparative results. It would have added great value to the paper if the authors compared with the technique of [10] (porting it to their target model) and confirmed experimentally the superiority of their proposed method. Although I understand that such comparison would have been time and work-consuming, it would have been very valuable."}

\blue{We agree that such a quantitative comparison is very valuable as it gives the results presented in our work a better context and value. Therefore, we have performed additional comparative experiments of our approach with SGD+M+QAS and MCUNet-5FPS~\cite{lin2022device}, which we present in a new section~\ref{sec:evaluation:mcunet}. The results show that (a) our optimizer slightly outperforms SGD+M+QAS when retraining MCUNet, and that more interestingly (b) our architecture MBedNet provides a much better tradeoff between memory, latency, and accuracy for on-device training than MCUNet-5FPS (ported to our framework) allowing not only inference at 5FPS but also training.}

\textit{"A more general issue related to all on-device learning libraries is the storage of input data. While it is not the main goal of the paper, which focuses on optimizing complexity and memory occupation for intermediate buffers, the issue should be at least mentioned/discussed. Otherwise the memory benefits of the proposed fully-quantized training could be nullified. In fact, in all experiments shown in this paper, the DNN is trained/fine-tuned for multiple epochs. This implies storing old data on-device (in a replay buffer) and feeding them to the network multiple times. This buffer could be, by far, the most dominant user of the system's memory. Continual learning techniques such as latent replay and others try to mitigate this issue, but once again, the authors should have at least mentioned them and discussed how their framework can be combined/complemented with those techniques."}

\blue{We thank the reviewer for raising the important issue of input "training" data storage, and have therefore added a paragraph to our manuscript to highlight this point more explicitly. As we mention in Sec.~\ref{sec:implementation:quant_bp}, our approach avoids to store and process entire mini-batches of input data in RAM by instead caching and accumulating weight gradients per layer. This allows us to store only a single input sample and label in RAM at a time, as it is sufficient to accumulate the resulting per-sample gradients in the gradient buffers of the layers until a full weight update step can be performed. Since it makes now difference to our method whether the DNN is in training or inference mode other than if the BP graph for a sample is executed or not, this implies even that a regular inference can be used interchangeably alongside the processing of samples used for training. We believe this feature is very helpful because at the edge, training data is often generated over time by a sensor or streamed in sample by sample over an external connection. In addition, we strongly agree that an evaluation of how our optimizer can be combined with more sophisticated continuous learning techniques is very interesting. We would consider this definitely as future work to extend on this paper.}

\blue{The RAM we report, for example, in Fig.~\ref{fig:retrain_results:memory_dynamic} includes both the RAM memory needed to hold all the gradient buffers and an input sample with its label. As a result, no additional memory is required to perform a training step beyond the values we report. To store larger chunks of training data over a longer period of time, e.g., in the form of a replay buffer as mentioned by the reviewer, we recommend using external memory to swap samples in and out of RAM as required. For example, for a demonstration of our method on an OpenMV MCU, we store a file with 2000 training samples and 500 evaluation samples of the animal dataset discussed in Fig.~\ref{fig:retrain_results} on a micro-SD card and swap them into RAM sample by sample using the MCU's SPI interface to facilitate training over multiple epochs. Of course, such an approach comes at the cost of additional delay due to the SPI interface.}

\textit{"There are no comments on the really high standard deviation in some cases of figure 4b. Especially for the last two plots of the figure. The value seems really high, differently for what is visible on almost all the other plots."}

\blue{To implement quantized layers, our method extensively uses SIMD instructions for arithmetic operations, which are available for integer types as part of ARM's DSP extension. The use of such SIMD instructions results in a significant speedup, especially compared to a floating-point based implementation where such instructions do not exist for Cortex-M MCUs, compare the high speedup between the blue and green bars in Fig.~\ref{fig:retrain_results:latency}. Now, the reason of why the mixed configuration, i.e., the orange bars, results in a similar latency as the fully quantized version, i.e., the blue bars, is that in the mixed configuration only the last layer, i.e., the linear classification head, is computed in floating-point, which is much less costly than the comparatively much more expensive initial convolutional layers of the CNNs, which in the mixed configuration are still computed in quantized form. All of the effects described above are amplified by the large input sizes of the cifar10 and cifar100 datasets (128x128x3 in our experiments, right bars in Fig.~\ref{fig:retrain_results:latency}), which resulte in even more computations in the already computationally expensive first convolutional layers compared to the much smaller input sizes of e.g. dalic and cwru (1x1024 and 1x512, left bars in Fig.~\ref{fig:retrain_results:latency}).}

\textit{"For both the MbedNet model and the smaller LeNet model used on MNIST, it would be better to show the exact hyperparameters (e.g. in a table or figure)."}

\blue{Thank you for pointing this out. Our optimizer has only two standard SGD hyperparameters, learning rate and batch size, which we set to learning rate 0.001 and batch size 48 for all our experiments. Therefore, we decided not to include a dedicated table or figure, but instead list the two hyperparameters and their values that we used to retrain LeNet, MbedNet, and MCUNet in Sec.~\ref{sec:evaluation} of our manuscript.}

\textit{"In Sec. IV the authors mention that they prune the network, but they should describe which pruning algorithm is used, and perhaps add a reference."}

\blue{We used an iterative pruning schedule with an $L1$-norm heuristic and automated gradual pruning. We have added this clarification to the manuscript. We want to emphasize that the use of pruning is not required for the training approach we discuss in this paper to be effective, but can instead be used orthogonally to reduce the memory and computational overhead of layers that are not retrained on-device.}

\subsection{Review \#51C}

\textit{"Novelty is limited.
The contributions are not clear.
The discussion and takeaways from the paper's results are not clear.}

\textit{The paper lacks clear demonstration of contributions. As of now, the paper's main technical contributions seem to be the two methods described in section 3. However, the paper does not use these contribution items and compare against relevant state of the art in the evaluation section. Instead the paper uses these two methods only as potential improvement methods and demonstrate the tradeoff between accuracy vs. latency/energy on three different microcontrollers."}

\blue{The novelty of our approach is a method for on-device training on Cortex-M MCUs that can overcome the challenges posed by the memory, computational, and bandwidth constraints of these highly resource- and performance-limited systems. For the convenience of the reviewer, we summarize here again the four main contributions and claims of our work, which can be found in Sec.~\ref{sec:contribution} of our manuscript.
\begin{enumerate}
    \item A novel, fully quantized, memory-efficient DNN optimizer to enable on-device training on MCUs, which can achieve accuracy similar to regular floating-point optimizers through gradient standardization.
    \item A memory-efficient version of stochastic gradient descent with support for arbitrarily large minibatches at no additional memory cost.
    \item An online per-sample partial gradient updating strategy that dynamically reduces the number of structures in tensors for which gradients need to be computed based on a magnitude-based selection heuristic, thereby reducing computational complexity with minimal impact on training performance.
    \item A comprehensive evaluation and analysis of the performance of our method, including latency and energy measured on real hardware, and a discussion of the resulting tradeoffs in the context of three Cortex-M MCUs of different sizes (Cortex-M0+, Cortex-M4, Cortex-M7).
    \item A comparison with SGD-M-QAS and MCUNet-5FPS as a novel contribution of this rebuttal.
\end{enumerate}}

\blue{As a result, a major claim and message of our work is that fully quantized training can be extended to enable on-device training of arbitrary CNN architectures on Cortex-M MCUs for datasets of different type and complexity by carefully considering the tradeoff between the number of layers to train, accuracy after retraining, memory, energy, and latency.}

\blue{Finally, agreeing with the reviewer that a comparison of our method with relevant state-of-the-art techniques was missing we have added an additional section to our evaluation, see Sec.~\ref{sec:evaluation:mcunet}, where we present and discuss additional comparative experiments of our approach with MCUNet-5FPS and SGD+M+QAS~\cite{lin2022device}. The results show that our optimizer was able to slightly improve the retraining results achieved by SGD+M+QAS, and that our MBedNet architecture provides a better tradeoff between resource requirements and accuracy for retraining than MCUNet. The new additional experiments, together with the accuracy vs. latency/energy tradeoffs presented in our evaluation, provide a more comprehensive insight into the performance and flexibility of our method in the context of the current state-of-the-art.}
